Are Your Reviewers Being Treated Equally? Discovering Subgroup Structures to Improve Fairness in Spam Detection

User-generated reviews of products are vital assets of online commerce, such as Amazon and Yelp, while fake reviews are prevalent to mislead customers. GNN is the state-of-the-art method that detects suspicious reviewers by exploiting the topologies of the graph connecting reviewers, reviews, and target products. However, the discrepancy in the detection accuracy over different groups of reviewers can degrade reviewer engagement and customer trust in the review websites. Unlike the previous belief that the difference between the groups causes unfairness, we study the subgroup structures within the groups that can also cause discrepancies in treating different groups. This paper addresses the challenges of defining, approximating, and utilizing a new subgroup structure for fair spam detection. We first identify subgroup structures in the review graph that lead to discrepant accuracy in the groups. The complex dependencies over the review graph create difficulties in teasing out subgroups hidden within larger groups. We design a model that can be trained to jointly infer the hidden subgroup memberships and exploits the membership for calibrating the detection accuracy across groups. Comprehensive comparisons against baselines on three large Yelp review datasets demonstrate that the subgroup membership can be identified and exploited for group fairness.

==> appendices.tex <==
\section{Appendix}
\begin{table*}
    \centering
    \small 
    % \setlength{\abovecaptionskip}{-0.05cm}
    \caption{NDCG values for the outputs of spam detectors on three Yelp datasets.
    Shown are the average results over all different splits.
    ``\textbf{\textcolor{red}{*}}'' denotes our method. \textcolor{red}{Add that the lower the metric the better.}}
    % \setlength{\tabcolsep}{12pt}{
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c c c | c c c |c c c}
    \toprule
        \textbf{Detector} & \textbf{NDCG(\%)} & \multicolumn{3}{c|}{\textbf{Chi}} & \multicolumn{3}{c|}{\textbf{NYC}} & \multicolumn{3}{c}{\textbf{Zip}} \\  
         \cline{1-11}
        \multirow{3}*{\textbf{FairGNN}~\cite{dai2021say}} & $\mathcal{V}^R$ & \multicolumn{3}{c|}{86.2\tiny{$\pm $0.1}} & \multicolumn{3}{c|}{85.9\tiny{$\pm $0.0}}  & \multicolumn{3}{c}{89.6\tiny{$\pm $0.5}} \\
        ~ & $\mathcal{V}^R_1$ & \multicolumn{3}{c|}{86.2\tiny{$\pm $0.1}} & \multicolumn{3}{c|}{86.0\tiny{$\pm $0.0}}  & \multicolumn{3}{c}{89.6\tiny{$\pm $0.4}} \\
        \rowcolor{gray!20}
         \cellcolor{white} ~ & $\Delta_{\text{NDCG}}$ & \multicolumn{3}{c|}{53.7\tiny{$\pm $2.1}} & \multicolumn{3}{c|}{20.7\tiny{$\pm $1.1}} & \multicolumn{3}{c}{36.4\tiny{$\pm $4.6}} \\
        \cline{1-11}
         \multirow{3}*{\textbf{EDITS}~\cite{dong2022edits}} & $\mathcal{V}^R$ & \multicolumn{3}{c|}{84.3\tiny{$\pm $0.3}} & \multicolumn{3}{c|}{84.9\tiny{$\pm $0.1}} & \multicolumn{3}{c}{89.2\tiny{$\pm $0.0}} \\
          ~ & $\mathcal{V}^R_1$ & \multicolumn{3}{c|}{84.3\tiny{$\pm $0.3}} & \multicolumn{3}{c|}{85.1\tiny{$\pm $0.1}} & \multicolumn{3}{c}{89.3\tiny{$\pm $0.0}}\\
        \rowcolor{gray!20} 
         \cellcolor{white} ~ & $\Delta_{\text{NDCG}}$ & \multicolumn{3}{c|}{50.9\tiny{$\pm $2.3}} & \multicolumn{3}{c|}{32.7\tiny{$\pm $1.5}} & \multicolumn{3}{c}{39.4\tiny{$\pm $10.6}} \\
        \cline{1-11}
        \midrule
          \multirow{2}*{\textbf{Detector}}&  \multirow{2}*{\textbf{NDCG(\%)}}  & \multicolumn{3}{c|}{\textbf{GNN}$(g_{\boldsymbol{\theta}})$} & \multicolumn{3}{c|}{\textbf{GNN}$(g_{\boldsymbol{\theta}})$} & \multicolumn{3}{c}{\textbf{GNN}$(g_{\boldsymbol{\theta}})$}\\
         &   ~&  \textbf{w/o} & \textbf{Pre-trained} &  \textbf{Joint\textcolor{red}{*}}& \textbf{w/o} & \textbf{Pre-trained} &  \textbf{Joint\textcolor{red}{*}} & \textbf{w/o} & \textbf{Pre-trained} &  \textbf{Joint\textcolor{red}{*}}\\
         \cline{1-11}
     \multirow{3}*{\textbf{GNN}} &  $\mathcal{V}^R$ & 84.5\tiny{$\pm$0.9}  & 83.2\tiny{$\pm $1.5} & 83.3\tiny{$\pm $2.2}  & 85.2\tiny{$\pm $0.8} & 85.1\tiny{$\pm$0.8} &  85.2\tiny{$\pm$0.5} & 88.4\tiny{$\pm$1.4} & 87.6\tiny{$\pm$1.5} & 88.6\tiny{$\pm$1.0}\\    
        ~ & $\mathcal{V}^R_1$ & 84.7\tiny{$\pm $0.9} & 83.5\tiny{$\pm $1.3} & 83.6\tiny{$\pm $2.1} & 85.1\tiny{$\pm$ 0.8} & 85.3\tiny{$\pm$0.8} & 85.2\tiny{$\pm$0.5} & 88.4\tiny{$\pm$1.4} & 87.6\tiny{$\pm$1.5} & 88.6\tiny{$\pm$1.0}\\
      \rowcolor{gray!20} 
     \cellcolor{white} ~ & $\Delta_{\text{NDCG}}$ & 51.2\tiny{$\pm $2.1} & 51.0\tiny{$\pm $3.0} & \textbf{50.7}\tiny{$\pm $3.5}  & 21.9\tiny{$\pm$7.0} & 21.8\tiny{$\pm$7.8} & \textbf{21.3}\tiny{$\pm$8.9} &  36.3\tiny{$\pm$10.4} & \textbf{34.3}\tiny{$\pm$10.8} &  34.8\tiny{$\pm$11.1}\\     % delta ndcg
     \cline{1-11}
         \multirow{3}*{\textbf{GNN-}$\mathbf{S_{1}^{\textbf{Tr}}}$\textbf{\textcolor{red}{*}}} &  $\mathcal{V}^R$ & 85.6\tiny{$\pm $0.7} & 85.8\tiny{$\pm $0.5} & 85.6\tiny{$\pm $0.8}  & 85.8\tiny{$\pm$0.1} & 85.9\tiny{$\pm$0.0} &  85.9\tiny{$\pm$0.0} &  89.7\tiny{$\pm$0.2} & 89.7\tiny{$\pm$0.1} & 89.6\tiny{$\pm$0.1}\\
      ~  & $\mathcal{V}^R_1$ & 85.6\tiny{$\pm $0.7} & 85.8\tiny{$\pm $0.5} & 85.7\tiny{$\pm $0.8}  & 85.9\tiny{$\pm$0.0} & 86.0\tiny{$\pm$0.0} & 86.0\tiny{$\pm$0.0} & 89.7\tiny{$\pm$0.2} & 89.7\tiny{$\pm$0.1} & 89.6\tiny{$\pm$0.1}\\
       \rowcolor{gray!20}
     \cellcolor{white}  ~ & $\Delta_{\text{NDCG}}$ & 51.6\tiny{$\pm $0.9} & 50.3\tiny{$\pm $1.0} & \textbf{50.1}\tiny{$\pm $1.0}  & 19.1\tiny{$\pm$5.5} & 19.0\tiny{$\pm$5.2} & \textbf{17.9}\tiny{$\pm$6.1} & 38.7\tiny{$\pm$7.2} & 36.0\tiny{$\pm$9.0} & \textbf{34.3}\tiny{$\pm$11.5}\\ % delta ndcg
 \cline{1-11}
       \multirow{3}*{\textbf{GNN-}$\mathbf{S_{0}^{\textbf{Te}}}$} &  $\mathcal{V}^R$ & 85.1\tiny{$\pm $0.7} & 85.3\tiny{$\pm $1.4} & 85.2\tiny{$\pm $1.4} & 85.3\tiny{$\pm$0.6} & 85.4\tiny{$\pm$0.5} & 85.4\tiny{$\pm$0.4} &  89.4\tiny{$\pm$0.6} & 89.6\tiny{$\pm$0.1} & 89.0\tiny{$\pm$0.06} \\
       ~ & $\mathcal{V}^R_1$ & 85.2\tiny{$\pm $0.8} & 83.4\tiny{$\pm $1.3} & 83.5\tiny{$\pm $1.3} & 85.2\tiny{$\pm$0.6} & 85.5\tiny{$\pm$0.4} & 85.5\tiny{$\pm$0.4} & 89.4\tiny{$\pm$0.06} & 89.0\tiny{$\pm$0.01} & 89.1\tiny{$\pm$0.06}\\
       \rowcolor{gray!20}
       \cellcolor{white} ~ & $\Delta_{\text{NDCG}}$ & 51.2\tiny{$\pm $1.5} & 
       \textbf{50.9}\tiny{$\pm $2.4} & \textbf{50.9}\tiny{$\pm $2.3}  & 21.9\tiny{$\pm$6.9}  & 21.9\tiny{$\pm$6.3}  & \textbf{20.9}\tiny{$\pm$9.4} & 38.9\tiny{$\pm$7.6} & 36.9\tiny{$\pm$9.5} & \textbf{34.9}\tiny{$\pm$11.0}\\   % delta ndcg
 \cline{1-11}
        \multirow{3}*{\textbf{GNN-}$\mathbf{S_{1}^{\textbf{Te}}}$} &  $\mathcal{V}^R$ & 84.7\tiny{$\pm $1.3} & 83.7\tiny{$\pm $0.9} & 83.1\tiny{$\pm $0.9}  & 85.7\tiny{$\pm$0.1} & 85.8\tiny{$\pm$0.1} & 85.8\tiny{$\pm$0.2} &  89.6\tiny{$\pm$0.3} & 89.6\tiny{$\pm$0.1} & 89.5\tiny{$\pm$0.3} \\
       ~ & $\mathcal{V}^R_1$ & 84.8\tiny{$\pm $1.3} & 83.9\tiny{$\pm $0.9} & 83.4\tiny{$\pm $0.9} & 85.8\tiny{$\pm$0.1} & 85.8\tiny{$\pm$0.1} & 85.8\tiny{$\pm$0.1} & 89.6\tiny{$\pm$0.3} & 89.6\tiny{$\pm$0.1} & 89.5\tiny{$\pm$0.3}\\
       \rowcolor{gray!20}
       \cellcolor{white} ~ & $\Delta_{\text{NDCG}}$ & 51.3\tiny{$\pm $0.6} & 50.8\tiny{$\pm $0.6} & \textbf{50.2}\tiny{$\pm $1.0}  &  21.0\tiny{$\pm$5.4}  & 19.8\tiny{$\pm$5.4}  & \textbf{19.3}\tiny{$\pm$6.8} & 38.7\tiny{$\pm$7.2} & 36.2\tiny{$\pm$9.5} & \textbf{34.6}\tiny{$\pm$11.4}\\   % delta NDCG
    \bottomrule
    \end{tabular}}
    \label{tab: big table}
    % \vspace{-0.5cm}
\end{table*}
